Photo-dynamical Analysis of Circumbinary Multi-planet system TOI-1338: a Fully Coplanar Configuration with a Puffy Planet

TOI-1338 is the first circumbinary planet system discovered by TESS. It has one transiting planet at P$\sim$95 day and an outer non-transiting planet at P$\sim$215 day complemented by RV observation. Here we present a global photo-dynamical modeling of the TOI-1338 system that self-consistently accounts for the mutual gravitational interactions between all known bodies in the system. As a result, the three-dimensional architecture of the system can be established by comparing the model with additional data from TESS Extended Mission and published HARPS/ESPRESSO radial velocity data. We report an inconsistency of binary RV signal between HARPS and ESPRESSO, which could be due to the contamination of the secondary star. According to stability analysis, the RV data via ESPRESSO is preferred. Our results are summarized as follows: (1) the inner transiting planet is extremely coplanar to the binary plane $\Delta I_b \sim 0.12 ^\circ$, making it a permanently transiting circumbinary planet at any nodal precession phases. We updated the future transit ephemerides with improved precisions. (2) The outer planet, despite its non-transiting nature, is also coplanar with the binary plane by $\Delta I_c=9.1^{+6.0 \circ}_{-4.8}$ (22$^\circ$ for 99\% upper limit). (3) The inner planet could have a density of $0.137 \pm 0.026$ g/cm$^{-3}$. With a TESS magnitude of 11.45, TOI-1338 b is an optimal circumbinary planet for ground-based follow-up and transit spectroscopy.

==> referee_report.tex <==

Reviewer:
The paper integrates the recently published RVs of TOI 1338 with an analysis of previously unpublished transits of planet TOI 1338 b, for a significantly improved characterisation of the TOI-1338 planet system. The methodology and interpretation of the results are presented in a very clear and straightforward manner, using state-of the art analysis tools, and the results appear to be reliable. Publication is therefore recommended after minor modifications, outlined below.

While the redaction is clear and in general well understandable, the text contains many minor grammar errors (like many missing 'the's ); a grammar revision should therefore be performed. In the detailed comments below, only some of such corrections are indicated, mostly when the understandability of the text was affected.


L=line

Since the RVs are essential in this work, a short overview over the RV dataset used in the analysis should be given. In particular, the number of RV points of each data-set used in the analysis should be given. It is also of note that S23's Tables 3-5 have numerous RV points with flags, so it should be stated which of these were used. This could be done in the introduction (e.g. after mention of S23 in L35), or in a separate sub-section. 

L25: system stability limit -> system inner stability limit 

L33: ... is the second circumbinary multiplanet system [add:] around a main-sequence binary  
(several more multiplanet CBP systems detected by ETVs are known, but around evolved stars)

L34: TOI-1338 b was discovered by TESS photometry (Kostov et al. 2020, hereafter K20).[add:] from transits in Sectors 3, 6 and 10 (this should be stated, in order to know which are the newly analysed data in your work)


L65: 54.1" and 58.9"

L68: SOAR speckle imaging is mentioned; give reference and a few-word-long description of instrument 

L76 has a dump -> has a fall-off 

L88: Regarding the parameter set used with batman: It is apparent that the value of the semi-major axis a will not be a correct, due to the lateral motion of the eclipsed binary-component. However, as I understand, the output from these fits can be treated as virtual set of parameters, since the aim of the fit has been the determination of the transit mid-time and duration. A brief description of the calculation of the transit-durations in Table 1 should therefore be given.

L94 "The flux errors are also reScaled (missing S)...": Are these the Error inflation factors in Table 1? Please clarify

Also to Table 1: The uncertainties of the observed midtimes should be given in days, to be comparable to the values given in the column 'Predicted Midtime'


On the parameter set used in Sect 3.1 and given in Table 2, several comments:
i) For the binary, a Mean Anomaly ('M.A.bin') is given, whereas for the planets, mean longitudes (lambda) are given. These should be converted to give either
the mean anomalies or mean longitudes for all objects. 

ii) In any case, the mean anomaly 'M.A. bin' can refer to only one of the binary components , since the other one is offset by 180 deg. So, it should likely be labelled as MA_A. (or lambda_A if you convert to mean longitude). The same goes for omega_bin. 

iii) The epoch of reference for the mean anomalies/mean longitudes should be clearly stated in the table (e.g. as a footnote to it); currently it is rather hidden in the text at L151. 

L125: Setting the limb-darkening coefficients of the secondary to be same ones as the primary is a poor choice, since these are rather different, a solar-like star and an M-dwarf, with very different LD-coefficients. Better would have been the use of fixed LD coefficients for the secondary, using typical values for such a star; best are the tabulations by Claret 2018, A&A 618, id.A20. In any case, given the low S/N of the secondary eclipses, the choice of LD coefficients for the secondary is not of relevance. A statement in that sense should be added therefore.  

L154: a 'stability limit' in the initial parameters for the outer planet is mentioned. It is not apparent what this stability limit is about, since the outer planet is far away from the inner orbital stability limit, and to my knowledge, there are no stability limits for mutual orbital inclinations (if there are, these should be cited) 

( L199: Here the lack of not knowing the number of RV points became apparent. But as stated above, it would be best to mention them earlier in the text. )

L207: ... we assume constant zero >flux< dilution ...

L241: a reference for the whfast integrator should be given.

L246: (change): ...the larger the eccentricity e_c of TOI-1338 c is,...

L253: untransiting -> non-transiting

L277: In Section 4.2 and onwards, masses and radii of the planets are discussed in both Jupiter and Earth units. Either Jupiter or Earth units should be used consistently in the whole work (If Earth units are used, also convert values in Table 2)

L281: However, the mass constraints remain -> However, the mass obtained for planet b remains...

L285: that the mass constraints reported -> that the masses reported 

L291-294: Starting with 'We also show', the authors should attempt to rewrite this text to be better understandable.

Fig 6 caption: Black error bars -> Black symbols with error bars 
Also, '11 binned RVs' : are these RVs binned over 11 phased data points? Or are these binned over 11 uniform phase-segments (hence with different numbers of RVs in each bin)? This should be specified more clearly. 

Fig 7 caption: 'tweaked model' -> best-fit model (if this is correct). Also: interacted -> interacting

L317: TTVs and TDVs if we -> TTVs and TDVs in models in which we

L323, eq (1): add a suffix 'c' to Delta I.

L327, 345 and 351: DeltaI (upper case I, in order to be consistent with Table 2 and other occurrences of the mutual inclination in the text)

L328: of additional fit>s<, with ic >being fixed< between 50 and 130 (if it is correct that I_c and Omega_c was fixed)

L328: All >other< parameters are fixed...

L332: except that >binary< eclipse light curves (if this is correct)

L361: The transmission spectroscopy metric (TSM) for planet b should be calculated, see Kempton+ 2018. S23 got a value of 39 and already states: " a lower mass would imply a larger scale height and therefore a significantly larger TSM." ; so knowing this higher value is of interest.

Fig 10: It should be stated that the right plots show two periods of the RVs folded by the binary period (if this is correct)

The reference of S23 needs to be actualised, it is now a Nature Astronomy paper

Data Editor's Review:
One of our expert data editors has reviewed your initial manuscript submission and has the following suggestion(s) to help improve the data, software citation and/or overall content. Please treat this as you would a reviewer's comments and respond accordingly in your report to the science editor. Questions can be sent directly to the data editors at data-editors@aas.org.


==> response_to_referee.tex <==

Dear Prof. Endl,

We thank the referee for a careful read and the constructive comments! We have revised the manuscript following suggestions from the referee. We append below our response to the referee's report.  

In our response, we respond to each comment, describe edits to figures and tables (collected at the end but in response to comments from the referee), and end with additional revisions we made to the manuscript. We also edited the paper, with all substantive (not grammar) revisions boldfaced.

Mu-Tian Wang and Hui-Gen Liu


_____

=============================
Main Text Revisions
=============================

Section 2.1

- REVIEWER: SOAR speckle imaging is mentioned; give reference and a few-word-long description of instrument 
- RESPONSE: we added a reference to the instrument.

Section 2.2

- REVIEWER: Regarding the parameter set used with batman: It is apparent that the value of the semi-major axis a will not be a correct, due to the lateral motion of the eclipsed binary-component. However, as I understand, the output from these fits can be treated as a virtual set of parameters, since the aim of the fit has been the determination of the transit mid-time and duration. A brief description of the calculation of the transit durations in Table 1 should therefore be given.
- RESPONSE: Thank you for highlighting this issue. We used the semi-major axis to estimate transit midtimes and durations, and the durations were calculated from the fitted parameters in a similar manner to transits around single-star systems. However, this approach provides only a first-order approximation. As you correctly pointed out, due to the lateral motion of the binary, the transits of circumbinary planets will be asymmetric, unlike those in single-star systems. We believe it is important to acknowledge this difference for transiting planets around single stars and in circumbinary environments, and we have added a footnote to this effect after the relevant sentence.
Additionally, we realized that including the semi-major axis as a fitted parameter was not ideal for midtime/duration fitting. Since we estimate the durations from fitted parameters using Equation 14 of Winn2010, which requires the knowledge of planet period. Deriving periods (in time unit) from the fitted semi-major axis (in length unit) relies on the assumption of the stellar mass, which was previously set to 1 Solar Mass — a potentially unreasonable assumption. Therefore, we have revised the midtime/duration fitting in Section 2.2, using a new parameter set (Tmid, P, a/R*, b, Rp/R*, q1, q2). We have listed the newly derived transit midtimes and durations in Table 1, and these changes are also reflected in the updated Figure 3. However, the differences between the old and new results are minimal and do not affect the remainder of the analysis.

- REVIEWER: "The flux errors are also reScaled (missing S)...": Are these the Error inflation factors in Table 1? Please clarify
- RESPONSE: The scaling factors are the error inflation factors in Table 1. We have clarified this in the text.

Section 3.1

- REVIEWER: Setting the limb-darkening coefficients of the secondary to be the same ones as the primary is a poor choice, since these are rather different, a solar-like star and an M-dwarf, with very different LD-coefficients. Better would have been the use of fixed LD coefficients for the secondary, using typical values for such a star; best are the tabulations by Claret 2018, A&A 618, id.A20. In any case, given the low S/N of the secondary eclipses, the choice of LD coefficients for the secondary is not of relevance. A statement in that sense should be added therefore.  
- RESPONSE: we thank the referee for this enlightening comment. Adopting the theoretical LD coefficients from Claret+2018 is a more sensible choice. In the case of our modeling, we found during the secondary eclipse the G-dwarf entirely occults the M-dwarf, therefore different LD coefficients will not alter the predicted depth of the secondary eclipse, except for the ingress/egress phase, the error in light curves is at most 10 ppm. However, as the referee pointed out, the secondary light curves are overall of low SNR (flux_err_obs = 200 ppm). Therefore, the model chi_sq of all secondary eclipses decreased ~0.5, which is negligible since the degree of freedom associated with a secondary eclipse is 2500+. We have added a footnote about this in the text, mentioning the Claret+2018 value and the general influence to our model.

REFEREE: a 'stability limit' in the initial parameters for the outer planet is mentioned. It is not apparent what this stability limit is about, since the outer planet is far away from the inner orbital stability limit, and to my knowledge, there are no stability limits for mutual orbital inclinations (if there are, these should be cited) 
- RESPONSE: this stability limit refers to the system-wide stability limit. Standing+23 performed a frequency-based stability analysis, finding the outer planet’s mutual inclination relative to the binary plane should not exceed 40 degrees (Supplement Figure 8 in their paper). We added text to direct interested readers to this figure.

Section 3.2

- REVIEWER: Since the RVs are essential in this work, a short overview over the RV dataset used in the analysis should be given. In particular, the number of RV points of each data-set used in the analysis should be given. It is also of note that S23's Tables 3-5 have numerous RV points with flags, so it should be stated which of these were used. This could be done in the introduction (e.g. after mention of S23 in L35), or in a separate sub-section. 
- RESPONSE: thank you for the advice, we have integrated a new sub-section (3.2-Fitted data) with a description of the data fed to the photo-dynamical model (TESS light curves and RVs).

Section 4.2

- REVIEWER: starting with 'We also show', the authors should attempt to rewrite this text to be better understandable.
- RESPONSE: we have rewritten this paragraph, it is now in Line 311-317.

Section 5

- REVIEWER: The transmission spectroscopy metric (TSM) for planet b should be calculated, see Kempton+ 2018. S23 got a value of 39 and already states: "A lower mass would imply a larger scale height and therefore a significantly larger TSM." ; so knowing this higher value is of interest.
- RESPONSE: we calculated the TSM of TOI-1338 b to be 86 +/- 17, and added a sentence about this in Line 411-413.

=============================
FIGURES
=============================

- REVIEWER: Fig 6 caption:  '11 binned RVs' : are these RVs binned over 11 phased data points? Or are these binned over 11 uniform phase-segments (hence with different numbers of RVs in each bin)? This should be specified more clearly. 
- RESPONSE: these are RVs binned in 11 evenly-spaced intervals within one planet period. We clarified this in the text.

- REVIEWER: Fig 7 caption: 'tweaked model' -> best-fit model (if this is correct). Also: interacted -> interacting
Response: ‘tweaked model’ should be the correct text. We want to use this figure to demonstrate if the mass and inclination are tweaked, the TTV pattern will change, which we can leverage to constrain the inclination of TOI-1338 c using the observed TTV of TOI-1338 b.

=============================
TABLES
=============================

Table 1
--------
- REVIEWER: The uncertainties of the observed midtimes should be given in days, to be comparable to the values given in the column 'Predicted Midtime'
- RESPONSE: Now the midtime uncertainties are integrated to the 'Transit Midtime' column in unit of days.

Table 2
--------
- REVIEWER: For the binary, a Mean Anomaly ('M.A.bin') is given, whereas for the planets, mean longitudes (lambda) are given. These should be converted to give either the mean anomalies or mean longitudes for all objects. 
- RESPONSE: we have changed to report the mean-longitude for all orbits.

- REVIEWER: In any case, the mean anomaly 'M.A. bin' can refer to only one of the binary components, since the other one is offset by 180 deg. So, it should likely be labeled as MA_A. (or lambda_A if you convert to mean longitude). The same goes for omega_bin. 
- RESPONSE: thank you for pointing out the potential confusion. We have changed the subscript from 'bin' to 'B' for binary-relevant parameters.

- REVIEWER: The epoch of reference for the mean anomalies/mean longitudes should be clearly stated in the table (e.g. as a footnote to it); currently it is rather hidden in the text at L151. 
- RESPONSE: the reference epoch of orbital elements in Table 2 is now noted below the table.

- REVIEWER: In Section 4.2 and onwards, masses and radii of the planets are discussed in both Jupiter and Earth units. Either Jupiter or Earth units should be used consistently in the whole work (If Earth units are used, also convert values in Table 2)
- RESPONSE: We have added values in Earth/Jupiter units of b/c’s mass and radius in the ‘Derived Parameter’ Table 2. Mass and radius mentioned in text are now all formatted in Earth units.

=========================
Additional Revisions
=========================

1. We added comments on the convergence of the joint, espresso-only, and harps-only analysis posteriors. They are in Line 177-178 and Line 191-194.

2. TESS is now scheduled to re-observe TOI-1338 in Year 7(https://tess.mit.edu/tess-year-7-observations/). We predict three primary transits of TOI-1338 will occur during the TESS revisit and add a sentence about this in Line 384-386.

3. In Section 5 Line 395-408, we added a more detailed discussion to place TOI-1338 b in contexts of known sub-Saturns, along with a new figure 10 to make clearer comparisons with them.

